Dynamical pathways for the interaction of O2, H2O, CH4, and CO2 with a-alumina surfaces: Density functional tight-binding calculations

In this study, we investigated the physisorption mechanisms of O2, H2O, CH4, and CO2 molecules on alumina and their effect on electronic properties. We employed quantum-classical molecular dynamics simulations and the self-consistent-charge density-functional tight-binding (SCC-DFTB) approach to dynamically model these mechanisms. Our results revealed the binding pathways of O, H, and C atoms in the various molecules to Al and O atoms at the top atomic layers of the alpha-alumina surface. We examined several adsorption sites and molecular orientations relative to Al-terminated and Ox-terminated alumina surfaces and found that the most stable physisorbed state on the Al-terminated surface is located above the Al atom, while the Ox-terminated state is found above the oxygen, resulting in enhanced optical adsorbance. The dissociation of CH4 into CH2+H2 after interaction with the surface resulted in hydrogen production, but with low adsorbate rates. While, O2 molecules primarily bond to the Al atoms, leading to the highest adsorbance rate among the other molecules. Our findings provide important insights into the physisorption mechanisms of molecules on alumina and their impact on electronic properties

==> sections/figures_tables.tex <==
%%%%  Fig 1
\begin{figure}
\centering
  \includegraphics[width=0.55\linewidth]{Figures/Fig1.png}
  \caption{Structure of an alpha alumina unit cell with 60 atoms (24 Al and 36 O) that was energy optimized by SCC-DFTB.  }
  \label{fig:fig1}
\end{figure}

%%%%% Fig 2
%\begin{figure}
%\centering
%  \includegraphics[width=0.55\linewidth]{Figures/molecules.png}
%  \caption{Optimized molecules used to calculate binding energies for 
%  O$_2$ in a), H$_2$O in b), CH$_4$ in c), and CO$_2$ in d). Computed distribution of the electron (wave function squared) for the HOMO 
%  ($e^+$--blue and $e^-$--green) is shown.}
%  \label{fig:fig2a}
%\end{figure}

%%%%% Fig 3
\begin{figure}
\centering
  \includegraphics[width=0.48\linewidth]{Figures/Fig2.png}
  \caption{Alumina surface used to calculate binding energies with 
  identified adsorbate sites considering aluminium and oxygen layers 
  at the top of the surface. Density of states are shown in c).  }
  \label{fig:fig2}
\end{figure}

%%%% Fig 4
\begin{figure}
\centering
  \includegraphics[width=0.6\linewidth]{Figures/Fig3.png}
  \caption{Physisorption of O$_2$ in a), H$_2$O in b), 
  CH$_4$ in c), and CO$_2$ in d) on the alumina surface 
  for Al--terminated by considering all adsorbate sites. 
  Molecular 
  orientation is included in the calculations}
  \label{fig:fig3}
\end{figure}


%%% Fig 5
\begin{figure}
\centering
  \includegraphics[width=0.6\linewidth]{Figures/Fig4.png}
  \caption{Binding energy results for physisorption paths for
  H$_2$O on alumina surface for Al--terminated a) and 
  Ox--terminated in b), considering all the adsorbate sites. 
  Two different 
  orientations are considered in the calculations}
  \label{fig:fig4}
\end{figure}



%%%%%%% Tab. 1
\begin{table}[h!]
 \caption{Binding energy, $E_b$ [eV]  and 
 energy surface $\gamma_{\rm phys}$ [eV/nm$^2$] 
 of alumina surface with different molecules}
  \begin{tabular}[htbp]{@{}lrr@{}}
    \hline
    \multicolumn{3}{c}{Al--terminated} \\
    \hline
    Molecule & $E_b$  & $\gamma_{\rm phys}$\\
    \hline
    O$_2$  & -2.03  & 0.85 \\
    H$_2$O & -1.94  & 0.82\\
    CH$_4$ & -0.25  & 0.11 \\
    CO$_2$ & -2.05  & 0.87 \\
    \hline
    \multicolumn{3}{c}{Ox--terminated} \\
     \hline
    Molecule & $E_b$ & $\gamma_{\rm phys}$\\
    \hline
    O$_2$  & -3.03  & 1.28 \\
    H$_2$O & -3.14  & 1.33 \\
    CH$_4$ & -0.53  & 0.22 \\
    CO$_2$ & -11.38 & 4.80 \\
    \hline
  \end{tabular}
  \label{tab:tab1}
\end{table}


%%%%%%%%%%%%%%%%%%%%
%%%% Fig 8
\begin{figure}
\centering
  \includegraphics[width=0.98\linewidth]{Figures/Publication4.png}
 % 
  \caption{Most stable adsorption 
configuration diagram and DOS results for the Al--terminated surface 
  with O$_2$ in a), H$_2$O in b), CH$_4$ in c), and CO$_2$ in d) at 
  the adsorbate site where $E_b$ is minimum. 
  We add a blue bar that represents the magnitude of the binding energy.  }
  \label{fig:fig6a}
\end{figure}

%%%%%%%% Fig 9
\begin{figure}
\centering
  \includegraphics[width=0.45\linewidth]{Figures/charge.png}
  \includegraphics[width=0.45\linewidth]{Figures/absorbance.png}
  \caption{The Mulliken charge of each atom of different molecules adsorbed 
  by the alumina surface is displayed in a) as a histogram, and Absorbance spectra 
  in b) of alumina with several molecules.
  CH$_4$ highly affects the charge distribution of the surface}
  \label{fig:fig7}
\end{figure}



%%%%%%%%%%%%%%%%%%%%
%%%% Fig 8
\begin{figure}
\centering
  \includegraphics[width=0.98\linewidth]{Figures/irradiation_results.png}
 % 
  \caption{Reflection and adsorbtion rates for different 
  emitting molecules at 1 eV on alumina surface. 
  Dissociation of molecules are observed during the 
  dynamics.}
  \label{fig:figRA}
\end{figure}


%%%%%%%%%%%%%%%%%%%%
%%%% Fig 8
\begin{figure}
\centering
  \includegraphics[width=0.98\linewidth]{Figures/Publication5.png}
 % 
  \caption{Final position of all adsorbed atoms after 1 eV 
  emition of  500 molecules of O$_2$ in a), H$_2$O in b), CH$_4$
  in c), 
  and CO$_2$ in d). Atoms and/or molecules are more likely 
  to be bond to an Al at the top layer of the surface.
  .  }
  \label{fig:islands}
\end{figure}


